Achievability and Impossibility of Exact Pairwise Ranking

We consider the problem of recovering the rank of a set of $n$ items based on noisy pairwise comparisons. We assume the SST class as the family of generative models. Our analysis gave sharp information theoretic upper and lower bound for the exact requirement, which matches exactly in the parametric limit. Our tight analysis on the algorithm induced by the moment method gave better constant in Minimax optimal rate than ~\citet{shah2017simple} and contribute to their open problem. The strategy we used in this work to obtain information theoretic bounds is based on combinatorial arguments and is of independent interest.

==> sections/exactdeter.tex <==
% \subsubsection{Impossibility}
% From the definition we know that the Bayes estimator $T_B^*$ is admissible in $\fk T$ on the Bayes risk given prior $\fk P$. This being said, the impossibility conditions of exact Bayesian pair-wise ranking is the condition under which no strongly consistent Bayes estimator with respect to prior $\fk P\in\ca P$ exists. We formalize this observation through the following claim that can be directly obtained from definition.
% \begin{claim}[Sufficient Conditions]
% For some prior $\fk P$, if the Bayes estimator cannot exactly rank then no other estimators exactly rank.
% \end{claim}
% To apply our analysis, we first define automorphism on the group of vertices in weighted directed graphs.

% % \begin{definition}[Automorphism in Weighted Directed Graphs]
% % We say an automorphism $\pi\in\bb P$ on a weighted directed graph $G(\ca V,\ca E)$ with $\ca V=[n]$ is a permutation on $\ca V$ such that the graph $ G^\prime$ permuted according to $\pi$ from $G$ is isomorphic to $G^\prime(\ca V^\prime,\ca E^\prime)$ with $\ca E=\ca E^\prime$. The automorphisms in specific graph $G$ formed an automorphism group, which we termed \texttt{Auto}(G). In particular, the non-identity permutation in \texttt{Auto}(G) is termed non-trivial automorphism.
% % \end{definition}
% However, in the deterministic comparison setting, the notion of indistinguishable pair acts in more importance in our analysis. Intuitively, the automorphism is too strong a requirement for the WDGs to fulfill.
% \begin{definition}[Indistinguishable Pair]\label{lm:4}
% We say the indistinguishable pair $(i,j)$ with $i,j\in[n]$ and $i\neq j$ is an unordered pair of indices in a graph $G(\ca V,\ca E)$ such that for the graph $G^\prime(\ca V^\prime,\ca E^\prime)$ where $\ca V=\ca V^\prime$ and $\ca E^\prime=\ca E\setminus\{(i,j),(j,i)\}$, there exists $\pi\in$\texttt{Auto}($G^\prime$) such that $\pi(i)=j\wedge\pi(j)=i$.
% \end{definition}
% The following lemma is the basis of our result, which we give in increasing generality.
% % \begin{fact}\label{fac1}
% % Let $\ca A^m=\sum_{i=1}^m\bfa A_{i}$, then if the weighted directed graph induced by $\ca A^m$ has a non-trivial automorphism $\pi$ with $\pi(i)=j$, $\pi(j)=i$ and $\pi(k)=k$ for all $k\in[n]\setminus\{i,j\}$ with $\Theta(1)$ probability, the Bayes estimator will fail the requirement of exact recovery.
% % \end{fact}
% % \begin{lemma}\label{lm22}
% % If there exists a indistinguishable pair with $\Theta(1)$ in $G(\ca V,\ca E)$, then the exact pairwise ranking will be impossible.
% % \end{lemma}
% % \begin{proof}
% % We denote the following events \begin{compactenum}
% % \item $A_1:\ca A_{i,j}^m\geq \ca A_{j,i}^m$
% % \item $A_2: \ca A_{i,j}^m< \ca A_{j,i}^m$
% % \item $A_3: \exists\pi\in\text{Auto}(G^\prime)\text{ s.t. }\pi(i)=\pi(j)$
% % \end{compactenum}
% % By the conditions given in the lemma, we directly see that
% % \begin{equation*}
% %     \bfa P(A_1|A_3)=\Theta(1)\;\;\;\bfa P(A_2|A_3)=\Theta(1)
% % \end{equation*}
% % Hence with probability at least $\min\{\bfa P(A_1,A_3),\bfa P(A_2,A_3)\}$, any estimator will make mistake, making the exact ranking impossible.
% % \end{proof}
% \textbf{Discussion:} Although the exact ranking is impossible, the almost exact ranking was not affected here, which will require a stronger condition to make 
% With more involved analysis, the above fact can be further extended with the help of the notion of disagreement between vertices. 
% \begin{definition}[Disgreement between vertices]
% Let $\ca A$ be the adjacency matrix of a WDG denoted by $G(\ca V,\ca E)$. Let $i,j,k\in\ca V$ with $i\neq j$. Then we say $i,j$ disagree on $k$ in $G$ if $\ca A_{i,k}\neq \ca A_{j,k}$ or $\ca A_{k,i}\neq\ca A_{k,j}$
% \end{definition}
% % \begin{lemma}
% % With the same notations in Fact 1, 
% %  let $G(\ca V,\ca E)$ be the graph induced by $\ca A^m$ with $\ca V=[n]$. If the a pair $(i,j)$ with $i\neq j$ and  $i,j$ disagree on at most $O\bigg( \frac{m\log\frac{1}{\gamma_{min}}}{{\log \frac{n}{\sqrt{m}} +m\log 4}}\bigg)$ vertices in $G$ with probability $\Theta(1)$, the Bayes estimator will fail the exact ranking. 
% % \end{lemma}
% % \begin{proof}
% % The idea is to show that when there exists a pair $(i,j)$ that disagrees on $\ca A^m$ by less than $s$ vertices with probability $\Theta(1)$, the probability of mistaking $i$ with $j$ by Bayes estimator in the graph will be $\Theta(1)$.

% % Let $\ca V(G)$ be the vertex set of $G$. Let $\{k:i,j \text{ disagree on } k\text{ and } k\in[n]\setminus\{i,j\}\}=\ca S$. Let $G^\prime$ be the subgraph with $\ca V(G^\prime)=\ca V(G)\setminus\ca S$.

% % Consider the event $E_1(\ca S)$: there exists an non-trivial automorphism $\pi:[n]\setminus \ca S\rightarrow[n]\setminus \ca S$ in graph $G^\prime$ with  $\pi(i)=j,\pi(j)=i$ and $card(\ca S)= s$.


% % We denote the event that an automorphism exists in the graph $G$ by $E_2$. We can then introduce the state space of $E_2|E_1(\ca S)$ by $\bb X(E_2|E_1(\ca S))\subset\{0,1\}^{2\times s\times m}$. For any elements $\bfa X_{k,r,t}\in\bb X(E_2|E_1)$ we have $\left\{\begin{matrix}
% % \ca S_j\text{ wins over }\ca S_r \text{ at round } t  & \text{ if } \bfa X_{1,r,t}=1 \\
% % \ca S_i\text{ wins over }\ca S_r \text{ at round } t  & \text{ if } \bfa X_{0,r,t}=1 \\
% % \end{matrix}\right.$ 
% % Then the following estimate can be obtained:
% % \begin{align*}
% %     \bfa P(E_2|E_1(\ca S))&\geq \sum_{\bfa X \in\bb X(E_2|E_1(\ca S))}\prod_{t\in[m]} F_{\pi^*(i),\pi^*(r)}^{\bfa X_{0,r,t}}(1-F_{\pstr i,\pstr r}^{1-\bfa X_{0,r,t}})F_{\pstr j,\pstr r}^{\bfa X_{1,r,t}}(1-F_{\pstr j,\pstr r})^{\bfa X_{1,r,t}}\\
% %     &=\Omega(card(\bb X(E_2|E_1(\ca S)))\gamma_{min}^{2m}))
% % \end{align*}
% % Then we obtain the cardinality of $\bb X(E_2|E_1)$ by a simple combinatorial asymptotically as :
% % \begin{equation*}
% %     card(\bb X(E_2|E_1(\ca S)))=\bigg(\sum_{i=1}^m\binom{m}{i}^2\bigg)^s=\bigg(\binom{2m}{m}\bigg)^s=\Theta\bigg(\frac{4^{ms}}{\sqrt{m}^s}\bigg)
% % \end{equation*}
% % Hence we have:
% % \begin{equation*}
% %     \bfa P(E_2|E_1(\ca S))=\Omega(\gamma_{min}^{2m}\cdot \frac{4^{ms}}{\sqrt{m}^s})
% % \end{equation*}
% % Hence, using marginalization, we have:
% % \begin{align*}
% %     \bfa P(E_2)&=\sum_{\ca S}\bfa P(E_2|E_1(\ca S))\bfa P(\ca S)\\&=\Omega\bigg(\binom{n-2}{s}\cdot\gamma_{min}^{2m}\cdot \frac{4^{ms}}{\sqrt{m}^s}\bigg)\\
% %     &=\Omega\bigg(\bigg(\frac{(n-2)e}{s}\bigg)^s\cdot\gamma_{min}^{2m}\cdot \frac{4^{ms}}{\sqrt{m}^s}\bigg)
% % \end{align*}
% % By letting the R.H.S, be $\Theta(1)$, we prove the statement in the lemma.
% % \end{proof}
% %     \Pi_{MAP}(\bfa A_1^m)&=\argmax_{\pi\in\bb P}
% %     \bfa P(\pa A(\pi,\Pi^*)=1|\bfa A_1^m)\\
% %     &\propto\argmax_{\pi\in\bb P}\bfa P(\bfa A_1^m|\pa A(\pi,\Pi^*)=1)\bfa P(\Pi^*=\pi)
% % \end{align*}
% % \begin{align*}
% %     \Pi_{MAP}&=\argmin_{\eta:\bb A\rightarrow\bb P}\bb E[\bfa 1_{\Pi^*\neq\eta(\bfa A_1^m)}]
% % \end{align*}
% % We are interested in the Bayes risk, stated as follows:

% % \begin{align*}
% %     \bfa P(\pa A(\Pi_{MAP}(\bfa A_1^m),\Pi^*)=1)
% % \end{align*}
% % A general principal for MAP estimator ensured its optimality under the exact ranking requirement, which is implied by its definition. In other words, MAP stays at the fundamental limits of exact ranking requirement, formalized through the following theorem:
% With the above lemmas we can give the following theorem, which found a inner point on the impossibility region.

% % \begin{theorem}
% % A Bayes estimator failed exact ranking if:
% %     \begin{align*}
% %   m=\Omega\bigg(\max\bigg\{\bigg(\frac{\gamma_{max}}{\gamma_{min}}\bigg)^{4n},\frac{\log n}{n(\log 2+3\log\frac{\gamma_{min}}{\gamma_{max}}+\log\gamma_{min})}\bigg\}\bigg)
% % \end{align*}
% % % and
% % % \begin{equation*}
% % %     \log\frac{1}{\gamma_{min}}=o\bigg (\frac{\log n}{mn}+\log 2-\frac{\log m}{4m}\bigg )
% % % \end{equation*}
% % % with $\gamma_{min}=\inf_{w_i,w_j}F(w_i-w_j)$ and $\gamma_{max}=\sup_{w_i,w_j}F(w_i-w_j)$ which also suggests that any other estimator will fail exact ranking. 

% % % Moreover, when
% % % \begin{equation*}
% % %     \log\frac{1}{\gamma_{max}}=\Omega\bigg (\frac{\log n}{mn}+\log 2-\frac{\log m}{4m}\bigg )
% % % \end{equation*}
% % % then there exists no distinguishable pair in the induced WDG a.s.
% % \end{theorem}

% % \begin{proof}
% % We denote the ensemble of $\bfa A^m_1$ by $\ca{ A}^m$, namely
% %  \begin{equation*}
% %      \ca {\bfa A}^m_{i,j}=\sum_{k=1}^m\bfa A_{i,j}^k
% %  \end{equation*}
% % %  We further let $a_{i,j}^m=\sum_{k=1}^m A^m_{i,j}$.
% % By the definition of prior measure and the independence between upper right entries given $\Pi=\pi^*$, we have
% % \begin{align*}
% %     \bfa P(\bfa A_1^m)&=\prod_{i,j\in [n]\wedge j>i}\bfa P(\ca A_{i,j}^m)\\
% %     &=\prod_{i,j\in [n]\wedge j>i}\binom{m}{\ca A_{i,j}^m}F_{\pstr i,\pstr i}^{\ca A_{i,j}^m}(1-F_{\pstr i,\pstr i})^{m-\ca A_{i,j}^m}
% % \end{align*}
% % According to the Lemma \ref{lm22}, as long as we find a sufficient condition under which automorphism exists with probability $\Theta(1)$, the Bayes estimator will fail in exact ranking. Let $G(i,j)$ be the graph induced by $\ca A_{i,j}^m$. Denote the event $E_{i,j}$ as the existence of non-trivial automorphism $\pi$ on $G(i,j)$ such that $\pi( i)=j$ and $\pi(j)=i$. 

% % We define the state space of $E_{i,j}$ as $\bb X(E_{i,j})\subset\{0,1\}^{n\times n\times (m+1)}$. $\forall\bfa X\in\bb X(E_{i,j})$, we denote:
% % $\bfa X_{k_1,k_2,k_3}=1$ if party $k_1$ wins over $k_2$ in the $k_3$-th comparison. The following statement holds:
% % \begin{align*}
% %     \bfa P(E_{i,j})&=\sum_{\bfa X\in\bb X(E_{i,j})}\prod_{k\in[n]\setminus\{i,j\}}\bfa P(\ca A_{i,k}^m=\ca A_{j,k}^m)\\
% %     &=\sum_{\bfa X\in\bb X(E_{i,j})}\prod_{k\in[n]\setminus\{i,j\}}\prod_{c\in[m]} F^{\bfa X_{i,k,c}}_{\pstr i,\pstr k}\cdot(1-F_{\pstr i,\pstr k})^{1-\bfa X_{i,k,c}}\\
% %     &F_{\pstr j,\pstr k}^{\bfa X_{j,k,c}}(1-F_{\pstr j,\pstr k})^{1-\bfa X_{i,k,c}}
% % \end{align*}
% % summing over $i,j$, we have
% % \begin{align*}
% %     \mu_n&=\sum_{\{i< j\}\wedge\{ i,j\in[n]\}}\sum_{\bfa X\in\bb X(E_{i,j})}\prod_{k\in[n]\setminus\{i,j\}}\prod_{c\in[m]} F^{\bfa X_{i,k,c}}_{\pstr i,\pstr k}\cdot(1-F_{\pstr i,\pstr k})^{1-\bfa X_{i,k,c}}\\
% %     &F_{\pstr j,\pstr k}^{\bfa X_{j,k,c}}(1-F_{\pstr j,\pstr k})^{1-\bfa X_{i,k,c}}
% % \end{align*}
% % Here we introduced the notation $\inf_{i\leq j}F_{i,j}=\gamma_{min}$, with $1-\gamma_{min}=\gamma_{max}$ being the minimum probability and maximum probability respectively. We then estimate the asymptotic rate of $\mu_n$. Ignoring constant factors, the number of summands is roughly
% % \begin{equation*}
% %     \Omega( n^2\cdot card(\bb X(E_{i,j}))\gamma_{min}^{2mn})
% % \end{equation*}
% % where 
% % \begin{align*}
% %     card(\bb X(E_{i,j}))&=\bigg(\sum_{i=0}^m\binom{m}{i}^2\bigg)^{n-2}=\bigg(\sum_{i=0}^m\binom{m}{i}\binom{m}{m-i}\bigg)^{n-2}\\
% %     &=\binom{2m}{m}^{n-2}=\Theta\bigg(\bigg(\frac{4^m}{\sqrt{m}}\bigg)^{n-2}\bigg)
% % \end{align*}
% % where we used the fact that the coefficient of $m$-th order term of the following polynomial 
% % $
% %     (1+x)^m(1+x)^m
% % $
% % is exactly the sum enclosed by the big bracket. This leads to 
% % \begin{equation*}
% %     \mu_n^2=\Omega\bigg(n^4\cdot\bigg(\frac{4^m}{\sqrt{m}}\bigg)^{2n-4}\gamma_{min}^{4mn}\bigg)
% % \end{equation*}

% % Then we discuss over the joint event of $E_{i,j}\cap E_{k,l}$. There are two types of joint events that are correlated. 
% % \begin{compactenum}
% % \item $card(\{i,j,k,l\})=3$. Without loss of generality, we denote the two pairs by $(i,j)$ and $(j,k)$. The event implies that for all $l\in[n]\setminus\{i,j,k\}$, $\ca A^m_{i,l}=\ca A^m_{j,l}=\ca A^m_{k,l}$ and $\ca A_{i,j}^m=\ca A_{k,j}^m$.
% % \item $card(\{i,j,k,l\})=4$. This condition implies that for all $o\in[n]\setminus\{i,j,k,l\}$, $\ca A^m_{i,o}=\ca A^m_{j,o}=\ca A^m_{k,o}=\ca A^m_{l,o}$ and $\ca A^m_{i,l}=\ca A^m_{i,k}=\ca A^m_{j,k}=\ca A^m_{j,l}$
% % \end{compactenum}
% % In the first regime, we can write the probability of joint events of regime 1 as:
% % \begin{align*}
% %     \bfa P(E_{i,j}\cap E_{j,k})&=\bfa P(\ca A^m_{k,j}=\ca A_{i,j}^m)\prod_{l\in[n]\setminus\{i,j,k\}}\bfa P(\ca A^m_{i,l}=\ca A^m_{j,l}=\ca A^m_{k,l})\\
% %     &=\big(\sum_{\bfa X\in\bb X(\ca A^m_{k,j}=\ca A_{i,j}^m)}\prod_{c\in[m]}F_{i,j}^{\bfa X_{i,j,c}}(1-F_{i,j})^{1-\bfa X_{i,j,c}}F_{k,j}^{\bfa X_{k,j,c}}(1-F_{k,j})^{1-\bfa X_{k,j,c}}\big)\\
% %     &\cdot\big(\prod_{l\in[n]\setminus\{i,j,k\}}\sum_{\bfa X\in\bb X(\ca A^m_{i,l}=\ca A^m_{j,l}=\ca A^m_{k,l})}\prod_{c\in[m]}F_{j,l}^{\bfa X_{j,l,c}}(1-F_{j,l})^{1-\bfa X_{j,l,c}}\\&
% %     F_{i,l}^{\bfa X_{i,l,c}}(1-F_{i,l})^{1-\bfa X_{i,l,c}}F_{k,l}^{\bfa X_{k,l,c}}(1-F_{k,l})^{1-\bfa X_{k,l,c}}\big)\\
% %     &=\Theta\bigg(\binom{2m}{m}\bigg(\sum_{i=0}^m\binom{m}{i}^3\bigg)^{n-3}\gamma_{max}^{2m+3m(n-3)}\bigg)\end{align*}
% %     Using the inequality that for $x_i\geq 1$ for all $i\in[n]$:
% %     \begin{equation*}
% %         (\sum_{i}^n x_i^2)^3\geq(\sum_{i}^nx_i^3)^2
% %     \end{equation*}
% %     we obtain that
% %     \begin{equation*}
% %         \sum_{i=0}^m\binom{m}{i}^3\leq\binom{2m}{m}^{3/2}
% %     \end{equation*}
% %     Hence
% %     \begin{equation*}
% %         \bfa P(E_{i,j}\cap E_{j,k})=O\bigg(\bigg(\frac{4^m}{\sqrt m}\bigg)^{1.5n-2.5}\gamma_{max}^{3mn-7m}\bigg)
% %     \end{equation*}
% % For the second case. we use similar method to estimate and obtain
% % \begin{align*}
% %     \bfa P(E_{i,j}\cap E_{k,l})&=\bfa P(\ca A^m_{i,l}=\ca A^m_{i,k}=\ca A^m_{j,k}=\ca A^m_{j,l})\cdot\prod_{o\in[n]\setminus\{i,j,k,l\}}\bfa P(\ca A^m_{i,o}=\ca A^m_{j,o}=\ca A^m_{k,o}=\ca A^m_{l,o})\\
% %     &=\bigg(\sum_{\bfa X\in\bb X(\ca A^m_{i,l}=\ca A^m_{i,k}=\ca A^m_{j,k}=\ca A^m_{j,l})}\prod_{c\in[m]}\ff{i,l}\ff{i,k}\\
% %     &\ff{j,k}\ff{j,l}\bigg)\\
% %     &\cdot\bigg(\prod_{o\in[n]\setminus\{i,j,k,l\}}\sum_{\bfa X\in\bb X(\ca A^m_{i,o}=\ca A^m_{j,o}=\ca A^m_{k,o}=\ca A^m_{l,o})}\prod_{c\in[m]}\ff{i,o}\\
% %     &\ff{j,o}\ff{k,o}\ff{l,o}\bigg)\\
% %     &=O\bigg(\bigg(\frac{4^m}{\sqrt m}\bigg)^{2n-6}\gamma_{max}^{4m+4m(n-4)}\bigg)
% % \end{align*}
% % Hence the $\gamma_n$ can be estimated by:
% % \begin{equation*}
% % \gamma_n=O\bigg(\binom{n}{3}\bigg(\frac{4^m}{\sqrt m}\bigg)^{1.5n-2.5}\gamma_{max}^{3mn-7m}+\binom{n}{4}\bigg(\frac{4^m}{\sqrt m}\bigg)^{2n-6}\gamma_{max}^{4mn-12m}  \bigg)
% % \end{equation*}
% % To have that $\gamma_n=O(\mu_n^2)$, we prove the above threshold.
% % \begin{align*}
% %     &\log(\frac{\gamma_{max}}{\gamma_{min}})=\Omega\bigg(\max\bigg\{\frac{2m\log 2-\log m +12m\log\gamma_{max}}{4nm},\frac{m\log2-0.25\log n+m\log\gamma_{min}}{3m}\bigg\}\bigg)
% % \end{align*}
% % % For the converse, using the first moment method we have
% % % \begin{equation*}
% % %     \mu_n=O\bigg(n^2\bigg(\frac{4^m}{\sqrt m}\bigg)^{n-2}\gamma_{max}^{2mn}\bigg)\rightarrow 0
% % % \end{equation*}
% % % or
% % % \begin{equation*}
% % %   \log\frac{1}{\gamma_{max}}=\Omega\bigg(\frac{\log n}{mn}+\log 2 -\frac{\log m}{4m}\bigg)
% % % \end{equation*}
% % % Then the automorphism will asymptotically exist.

% % \end{proof}


% % \begin{proof}
% % The proof of this lemma comes directly from the definition exact ranking. To guarantee exact ranking, MAP can only have $o(1)$ probability of error.
% % \end{proof}
% % Here we introduce a general definition of automorphism on weighted directed graphs


% % The above fact can be further relaxed to the following one:
% % \begin{lemma}\label{lm:3}
% % Let $\ca A^m(i,j)$ be the matrix that satisfies the following:
% % \begin{equation*}
% %     \ca A^m(i,j)_{k,l}=\left\{\begin{matrix}
% %  \ca A^m_{k,l}  &\text{ if } (k,l)\neq(i,j)\\
% %   0& \text{ if }(k,l)=(j,i) \\
% %   0&\text{ otherwise }
% % \end{matrix}\right.
% % \end{equation*}
% % Then the weighted directed graph induced by $\ca A^m(i,j)$ cannot be exactly ranked with MAP estimator if there exists an $\ca A^m(i,j)$m $i\leq j\wedge i,j\in[n]$ with $\Theta (1)$ probability.
% % \end{lemma}
% % \begin{proof}
% % We note that MAP will fail with $\Theta(1)$ probability on $\ca A^m(i,j)$
% % \end{proof}
% % The following lemma provides a general version of the above arguments.


% % \begin{fact}[Transitivity]
% % When $(i,j)$ and $(j,k)$ are indistinguishable pairs, $(i,k)$ is also an indistinguishable pair.
% % \end{fact}
% Our methodology is based on the following theorem.
% \begin{theorem}\label{thm:5}[Paley-Zygmund inequality] Let $X$ be a non-negative random variable. For all $0<\theta<1$,
% \begin{equation*}
%     \bfa P[X\geq\bb EX]\geq(1-\theta)^2\frac{(\bb EX)^2}{\bb E[X^2]}
% \end{equation*}
% \end{theorem}
% Taking $\theta\rightarrow 0$, the above theorem directly leads to
% \begin{corollary}\label{cor:3.1}Let $X$ be a non-negative random variable. Then
% \begin{equation*}
%     \bfa P(X>0)\geq\frac{(\bb EX)^2}{\bb E[X^2]}
% \end{equation*}
% \end{corollary}
% Then the following corollary comes directly from corollary~\ref{cor:3.1}
% \begin{corollary}
% Let $B_n=E_{1}\cup \cdots\cup E_{m(n)}$. where $E_{1},...,E_{m(n)}$ is a collection of events for each $n$. Write $i\overset{n}{\sim} j $ if $i\neq j$ and $E_{i}$ and $E_{j}$ are not independent. Then, letting
% \begin{equation*}
%     \mu_n:=\sum_{i=1}^{m(n)}\bfa P(E_{i}),\;\;\;\;\gamma_n:=\sum_{i\overset{n}{\sim}j}\bfa P(E_{i}\cap E_{j})
% \end{equation*}
% \label{cor1.2}
% where the second sum is over ordered pairs, we have $\lim_{n\rightarrow\infty}\bfa P(B_n)>0$ whenever $\mu_n\rightarrow\infty$ and $\gamma_n\leq C\mu_n^2$ for some $C>0$. If moreover $\gamma_n=o(\mu_n^2)$ then $\lim_{n\rightarrow\infty}\bfa P(B_n)=1$.
% \end{corollary}
% \begin{proof}
% Take $X:=X_n=\sum_{i=1}^{m(n)}\bfa 1_{E_i}$ in the previous theorem. We note that
% \begin{equation*}
%     Var[X_n]=\sum_{i}Var[\bfa 1_{E_i}]+\sum_{i\neq j}Cov[\bfa 1_{E_i},\bfa 1_{E_j}]
% \end{equation*}
% where we have
% \begin{equation*}
%     Var[\bfa 1_{E_i}]=\bb E[(\bfa 1_{E_i})^2]-(\bb E[\bfa 1_{E_i}])^2\leq\bfa P(E_i)
% \end{equation*}
% and, if $E_i$ and $E_j$ are independent,
% \begin{equation*}
%     Cov[\bfa 1_{E_i},\bfa 1_{E_j}]=0
% \end{equation*}
% whereas, if $i\overset{n}{\sim} j$,
% \begin{equation*}
%     Cov[\bfa 1_{E_i},\bfa 1_{E_j}]=\bb E[\bfa 1_{E_i}\bfa 1_{E_j}]-\bb E[\bfa 1_{E_i}]\bb E[\bfa 1_{E_j}]\leq\bfa P[E_i\cap E_j]
% \end{equation*}
% Hence,
% \begin{equation*}
%     \frac{Var[X_n]}{(\bb E X_n)^2}\leq\frac{\mu_n+\gamma_n}{\mu_n^2}=\frac{1}{\mu_n}+\frac{\gamma_n}{\mu_n^2}
% \end{equation*}
% and we note that
% \begin{equation*}
%     \frac{(\bb EX_n)^2}{E[X_n^2]}=\frac{(\bb EX_n)^2}{(\bb EX_n)^2+Var[X_n]}=\frac{1}{1+ \frac{Var[X_n]}{(\bb E X_n)^2}}
% \end{equation*}
% Applying the previous corollary yield the final result.
% \end{proof}

\subsubsection{Impossibility}

In this section, we denote $F_{i,j}$ as the event that $\bfa A_{i,k}^m>\bfa A_{j,k}^m$ for $k\in[n]\setminus\{i,j\}$ and denote $\bfa P_{i,j}=\bfa P(F_{i,j})$. Let $\bfa A\in\{0,1\}^{n\times n}$ denote the set of random variables in the state space where $\bfa A_{i,j}^m$ represents number of victory of party $i$ over $j$, when the number of comparisions toted $m$. In particular, we let $\bfa A_{i,i}=0$ for all $i\in[n]$, then the following lemma gives a necessary condition on exact ranking, connecting it to the standard hypothesis testing problem.

We first state a sufficient condition of impossibility.
\begin{lemma}\label{lm1}
For a pair of vertices $(i,j)$ with $i>j$, if $\bfa P(\bigcup_{i<j,i,j\in[n]}F_{i,j})=\Theta (1)$, then the Bayes estimator will fail the exact ranking.
\end{lemma}
% \begin{remark}
% Lemma 1 is a straight forward argument. In particular, if 
% \end{remark}
We then gave the Chernoff bound for the Binomial random variables.
\begin{lemma}\label{lm2}
For a binomial $X\sim Binom(n,p)$, when $k\leq np$, the tail inequality is given by Chernoff bound
\begin{align*}
    \bfa P(X\leq k)&=(n-k)\binom{n}{k}\int_{0}^{1-p}t^{n-k-1}(1-t)^kdt\leq\exp\bigg(-nD_{kl}\big(\frac{k}{m}\Vert p\big)\bigg)\\
    &\leq \exp(-2m\big(p-\frac{k}{m}\big)^2)
\end{align*}
\end{lemma}
Then we gave a lower bound on the difference between two binomials, stated by the following lemma
% \begin{proof}
% We define:
% \begin{align*}
%     V(m,p,q,x,y)=\binom{m}{x+y}\binom{m}{x}p^{x}q^{x+y}(1-p)^{m-x}(1-q)^{m-x-y}
% \end{align*}
% Then we have
% \begin{align*}
%     \log(V(m,p,q,x,y))&=\log\binom{m}{x+y}+\log\binom{m}{x}\\
%     &+x\log p+y\log q+(m-x)\log(1-p)+(m-x-y)\log(1-q)
% \end{align*}
% Then we use that for $k\leq N$
% \begin{align*}
%     \log\binom{N}{k}&\geq k\log N-\log k!-\log 4\\
%     \log k!&\leq(k+1)\log((k+1)/e)
% \end{align*}
% which gives
% \begin{align*}
%     \log\binom{N}{k}\geq k\log N-(k+1)\log(k+1)+k-\log 4
% \end{align*}
% and we have
% \begin{align*}
%     \log\binom{m}{x+y}&\geq (x+y)\log m-(x+y+1)\log (x+y+1)+x+y-\log 4\\
%     \log\binom{m}{x}&\geq x\log m-(x+1)\log(x+1)+x-\log 4
% \end{align*}
% Combining pieces, the following hold
% \begin{align*}
%      \log(V(m,p,q,x,y))&\geq (x+y)\log m+x\log m+ (m-x)\log(1-p)+(m-x-y)\log(1-q)\\
%                       &-(x+y+1)\log(x+y+1)-(x+1)\log(x+1)+x\log p+y\log q\\
%                       &+2x+y
% \end{align*}
% maximizing over $x,y$ we see that:
% \begin{align*}
%     \log\bfa P(X\geq Y)\geq \max_{x,y}\log (V(m,p,q,x,y))\geq
% \end{align*}
% \end{proof}
Then we review the Berry-Esseen theorem~\citep{berry1941accuracy}, which establishes the asymptotic rate of large deviation.
\begin{theorem}[Berry-Esseen]
Let $X_1,\ldots,X_n$ be independent random variables with the same distribution such that $
    \bb EX_j=0,\;\;\bb EX_j^2=\sigma^2>0,\;\;\bb E|X_j|^3<\infty$, Let $\rho=\frac{\bb E|X_j|^3}{\sigma^3}$ and
    \begin{equation*}
        \Phi(x)=\frac{1}{\sqrt{2\pi}}\int_{-\infty}^xe^{\frac{t^2}{2}}dt
    \end{equation*}
then, for any $n$, we have
\begin{align*}
    \sup_{x}\bigg|\bfa P\bigg\{\frac{1}{\sigma\sqrt{n}}\sum_{j=1}^nX_j\leq x\bigg\}-\Phi(x)\bigg|\leq A\frac{\rho}{\sqrt{n}}
\end{align*} 
where $A\leq 0.7655$ is the absolute positive constant.
\end{theorem}
% \begin{definition}[Stochastic domination]
% Let $\mu$ and $\nu$ be probability measures on $\bb R$. The measure $\mu$ is said to stochastically dominate $\mu$, denote by $\mu\succeq\nu$, if for all $x\in\bb R$
% \begin{equation*}
%     \mu[(x,+\infty)]\geq\nu[(x,+\infty)]
% \end{equation*}
% A real random variable $X$ stochastically dominates $Y$, denoted by $X\succeq Y$, if the law of $X$ dominates the law of $Y$.
% \end{definition}
% \begin{lemma}[Binomial is dominated by Poisson]
% When $\lambda\geq-\log(1-p)$, $Poi(m\lambda)$ stochastic-ally dominates $Binom(m,p)$
% \end{lemma}
The following lemma is a direct application of Berry-Esseen theorem.
\begin{lemma}\label{lm4}
Given a binomial $X\sim Binom(m,p)$, its c.d.f. can be estimated by:
\begin{align*}
    \sup_{x}\bigg|\bfa P(\bfa X\leq x)-\Phi(x)\bigg|\leq\frac{C_1}{\sqrt m}
\end{align*}
its p.d.f. can be estimated by
\begin{align*}
    \sup_x\bigg|\bfa P(\bfa X=x)-\frac{1}{\sqrt{2\pi p(1-p)m}}\exp\bigg(-\frac{(x-mp)^2}{p(1-p)m}\bigg)\bigg |\leq\frac{C_2}{\sqrt{m}}
\end{align*}
for some universal constant $C_1,C_2$ and $x\in\bb N$
\end{lemma}
By Berry-Esseen theorem and use the fact that Binomial random variables $\bfa X\sim Binom(m,p)$ can be seen as the ensemble of Bernoulli random variables $\bfa X=\sum_{i=1}^m\bfa x_i$ with $\bfa x_i\sim Bern(p)$ for all $i\in[m]$.
\begin{align*}
    \sup_{x}\bigg|\bfa P\bigg (\frac{1}{\sqrt{p(1-p)m}}(\bfa X-mp)\leq x\bigg )-\Phi (x)\bigg |\leq \frac{C_1}{\sqrt m}
\end{align*}
Or
\begin{align*}
    \sup_x\bigg|\bfa P(\bfa X\leq x)-\Phi\bigg (\frac{x-mp}{\sqrt{p(1-p)m}}\bigg )\bigg|\leq\frac{C_1}{\sqrt{m}}
\end{align*}
And we also have that for all $x\in\bb N$:
\begin{align*}
    &\bigg|\bfa P(\bfa X\leq x)-\bfa P(\bfa X\leq x-1)-\bigg(\Phi\bigg (\frac{x-mp}{\sqrt{p(1-p)m}}\bigg)-\Phi\bigg(\frac{x-1-mp}{\sqrt{p(1-p)m}}\bigg)\bigg)\bigg|\\
    &=\bigg | \bfa P(\bfa X=x)-\frac{1}{\sqrt{2\pi p(1-p)m}}\exp\bigg (-\frac{(x-mp)^2}{p(1-p)m}\bigg)\bigg |\leq\frac{C_2}{\sqrt{m}}
\end{align*}
where we already used the fact that
\begin{equation*}
    \frac{1}{\sqrt{2\pi p(1-p)m}}\bigg [\exp\bigg(-\frac{(x-mp)^2}{p(1-p)m}\bigg)-\exp\bigg(-\frac{(x-1-mp)^2}{p(1-p)m}\bigg)\bigg]\leq\frac{C_3}{\sqrt m}
\end{equation*}
% \begin{lemma}[Hoeffding's Bound on the difference between binomials]
% Given two random variables $X\sim Binom(m,p_1)$, $Y\sim Binom(m,p_2)$ Then the following holds for their difference:
% \begin{equation*}
%     \bfa P(X\leq Y)\leq\exp\bigg(-2\bigg(\frac{p_2(1-p_1)}{p_1(1-p_2)+p_2(1-p_1)} - \frac 12\bigg)^2 \big(p_1(1-p_2) + p_2(1-p_1)\big) m\bigg)
% \end{equation*}
% \end{lemma}
Then we review the Paley-Zygmund inequality, which is stated as
\begin{lemma}[Paley-Zygmund]
For random variable $Z>0$, for $\theta\in(0,1)$ we have
\begin{align*}
    \bfa P(Z\geq\theta\bb E[Z])\geq(1-\theta)^2\frac{\bb E[Z]^2}{\bb E[Z^2]}
\end{align*}
And for general random variable, we have
\begin{align*}
    \bfa P(\exp(tZ)\geq\theta\bb E[\exp(tZ)])\geq(1-\theta)^2\frac{\bb E[\exp(tZ)]^2}{\bb E[\exp(2tZ)]}
\end{align*}
\end{lemma}


which directly implies
\begin{corollary}[Second Order Method]
$
\bfa P(Z\geq 0)\geq\frac{\bb E[Z]^2}{\bb E[Z^2]}
$
\end{corollary}
and further implies
\begin{corollary}
Let $B_n=E_{1}\cup \cdots\cup E_{m(n)}$. where $E_{1},...,E_{m(n)}$ is a collection of events for each $n$. Write $i\overset{n}{\sim} j $ if $i\neq j$ and $E_{i}$ and $E_{j}$ are not independent. Then, letting
\begin{equation*}
    \mu_n:=\sum_{i=1}^{m(n)}\bfa P(E_{i}),\;\;\;\;\gamma_n:=\sum_{i\overset{n}{\sim}j}\bfa P(E_{i}\cap E_{j})
\end{equation*}
\label{cor1.2}
where the second sum is over ordered pairs, we have $\lim_{n\rightarrow\infty}\bfa P(B_n)>0$ whenever $\mu_n\rightarrow\infty$ and $\gamma_n\leq C\mu_n^2$ for some $C>0$. If moreover $\gamma_n=o(\mu_n^2)$ then $\lim_{n\rightarrow\infty}\bfa P(B_n)=1$.
\end{corollary}
\begin{proof}
Take $X:=X_n=\sum_{i=1}^{m(n)}\bfa 1_{E_i}$ in the previous theorem. We note that
\begin{equation*}
    Var[X_n]=\sum_{i}Var[\bfa 1_{E_i}]+\sum_{i\neq j}Cov[\bfa 1_{E_i},\bfa 1_{E_j}]
\end{equation*}
where we have
\begin{equation*}
    Var[\bfa 1_{E_i}]=\bb E[(\bfa 1_{E_i})^2]-(\bb E[\bfa 1_{E_i}])^2\leq\bfa P(E_i)
\end{equation*}
and, if $E_i$ and $E_j$ are independent,
\begin{equation*}
    Cov[\bfa 1_{E_i},\bfa 1_{E_j}]=0
\end{equation*}
whereas, if $i\overset{n}{\sim} j$,
\begin{equation*}
    Cov[\bfa 1_{E_i},\bfa 1_{E_j}]=\bb E[\bfa 1_{E_i}\bfa 1_{E_j}]-\bb E[\bfa 1_{E_i}]\bb E[\bfa 1_{E_j}]\leq\bfa P[E_i\cap E_j]
\end{equation*}
Hence,
\begin{equation*}
    \frac{Var[X_n]}{(\bb E X_n)^2}\leq\frac{\mu_n+\gamma_n}{\mu_n^2}=\frac{1}{\mu_n}+\frac{\gamma_n}{\mu_n^2}
\end{equation*}
and we note that
\begin{equation*}
    \frac{(\bb EX_n)^2}{E[X_n^2]}=\frac{(\bb EX_n)^2}{(\bb EX_n)^2+Var[X_n]}=\frac{1}{1+ \frac{Var[X_n]}{(\bb E X_n)^2}}
\end{equation*}
Applying the previous corollary yield the final result.
\end{proof}
We have the following several technical lemmas
\begin{lemma}
Let $X\sim Binom(m,p)$ and $Y\sim Binom (m,q)$ with $p<q$ and suppose $m$ is large enough, we have 
\begin{align*}
    \bfa P(X\geq Y)=1-\Phi(x)\geq\bigg (\frac{x}{x^2+1}\bigg )\frac{1}{\sqrt{2\pi}}\exp(-\frac{x^2}{2}) 
\end{align*}
with $x=\sqrt{\frac{m(q-p)^2}{p(1-p)+q(1-q)}}$
\end{lemma}
\begin{proof}
Denote $\psi_X$ as the moment generating function of random variable $X-\bb E[X]$. By normal approximation, we have
\begin{align*}
    \psi_{X-Y}(t)=\psi_X(t)/\psi_Y(t)=\bigg(\frac{(1-p)e^{-pt}+pe^{(1-p)t}}{(1-q)e^{-qt}+qe^{(1-q)t}}\bigg)^m\rightarrow\exp\bigg(\frac{(p(1-p)-q(1-q))nt^2}{2}\bigg)
\end{align*}
Then we use the fact that $X-Y\sim N(m(p-q),m(p(1-p)+q(1-q)))=N(\mu(p,q),\sigma^2(p,q))$ and obtain that:
\begin{align*}
     \bfa P(X\geq Y)&=\bfa P(X-Y\geq 0)=1-\Phi\bigg(\sqrt{\frac{-m(p-q)^2}{p(1-p)+q(1-q)}}\bigg)+O(\frac{1}{\sqrt m})
\end{align*}
where $\Phi(x)=\frac{1}{\sqrt{2\pi}}\int_{-\infty}^x e^{-\frac{t^2}{2}}dt$ is the c.d.f. of standard normal distribution. The extra term error is given by Berry-Esseen theorem. Then we recall the lowerbound on the Gaussian tail that for all $x>0$, the following holds
\begin{align*}
    1-\Phi(x)\geq\frac{x}{x^2+1}\frac{1}{\sqrt{2\pi}}e^{-\frac{x^2}{2}}
\end{align*}
with the assumption that $m$ is very large, we finish the proof.
\end{proof} 

% \begin{lemma}\label{lm:88}
% Given two random variables $X\sim Binom(m,p_1)$, $Y\sim Binom(m,p_2)$. Assuming $p_1\geq p_2$, then the following holds:
% \begin{equation*}
%     \bb E[(Y-X)^2]\leq  m (p_1-p_2)+m(m-1)(p_1-p_2)^2
% \end{equation*}
% \end{lemma}
% \begin{proof}
% We denote $Y-X=\sum_{i=1}^m\sigma_m$ by a sum of $m$ random variables i.i.d. $\sigma_1$ induces the following probability measure:
% \begin{align*}
%   \sigma_1= \left\{\begin{array}{ll}
% 1 &\text{ with probability } p_2(1-p_1)  \\
% 0 &\text{ with probability } p_2p_1+(1-p_2)(1-p_1)  \\
% -1&\text{ with probability } p_1(1-p_2)\\
% \end{array}\right.
% \end{align*}
% And the moment generating function, when $\lambda\geq 0$, is given by 
% \begin{align*}
%     \phi_{\sigma}(\lambda)=\bb E[\exp(\lambda(\sigma))]&=p_2(1-p_1)\exp(\lambda)+p_1p_2+(1-p_2)(1-p_1)+p_1(1-p_2)\exp(-\lambda)\\&\leq\exp(-\lambda\bb E[\sigma]+\frac{1}{2}\lambda^2\zeta^2)
% \end{align*}
% By Taylor expansion until the second order, we obtain that
% \begin{equation*}
%     \bb E[\sigma]=p_1-p_2\;\;\zeta=\sqrt{(-2p_1p_2+p_1+p_2)-(p_1-p_2)^2}
% \end{equation*}
% Therefore the generative function of $Y-X$ can be bounded by:
% \begin{align*}
%     \phi_{Y-X}(\lambda)&=\bb E[\exp(\lambda(Y-X)]\\
%     &=\prod_{i=1}^m\bb E[\exp(\lambda\sigma_i)]\\
%     &=\sum_{i=1}^\infty\bb E[\sigma^i]\frac{\lambda^i}{i!}\\
%     &\leq\exp(-m\lambda\bb E[\sigma]+\frac{m}{2}\lambda^2\zeta^2)\\
%     &=\sum_{i=1}^\infty\frac{-\lambda^im^i\bb E[\sigma]^i}{i!}+\sum_{i=1}^\infty\frac{m^{i}\lambda^{2i}}{2^i(i)!}\zeta^{2i}
% \end{align*}
% Hence, by comparing the term on the r.h.s. and l.h.s., we can see that:
% \begin{equation*}
%     \bb E[(Y-X)^2]=m^2\bb E[\sigma]^2 +m\zeta^2\leq m (p_1+p_2-p_1p_2)+m(m-1)(p_1-p_2)^2
% \end{equation*}
% \end{proof}

\begin{lemma}
\label{lm10}
Let $\bfa X\sim Binom(m,p_1),\bfa Y\sim Binom(m,p_2),\bfa Z\sim Binom(m,p_3)$. Assuming $p_1<p_2<p_3$ and $m$ is large, then 
\begin{align*}
    \bfa P(\bfa X>\max\{\bfa Y,\bfa Z\})&\leq(1+8p_1(1-p_1))^{-\frac{1}{2}}\exp\bigg(-m(\frac{1}{2}p_1^2+2p_2^2+2p_3^2)+\frac{(-1-2p_3-2p_2)^2}{4\frac{1+8p_1(1-p_1)}{2mp_1(1-p_1)}}\bigg)
\end{align*} 
\end{lemma}
\begin{proof}
Using lemma \ref{lm2} and \ref{lm4}, we divide the range $\{1,\ldots,m\}$ into $\{1,\ldots,\lfloor\min\{p_2,p_3\}\rfloor\}$, $\{\lfloor\min\{p_2,p_3\}\rfloor+1,\ldots,\lfloor\max\{p_2,p_3\}\rfloor\}$, and $\{\lfloor\max\{p_2,p_3\}\rfloor+1,\ldots,m\}$ and upper bound them separately.
Also, using the normal approximation and Berry Esseen, when $y\leq mp_2$ and $z\leq mp_3$, the following holds.
\begin{align*}
    \bfa P(\bfa Y\leq y)&\leq \exp\bigg (-\frac{(y-mp_2)^2}{2mp_2(1-p_2)}\bigg)+O(\frac{1}{\sqrt m})\\
    \bfa P(\bfa Z\leq z)&\leq\exp\bigg(-\frac{(z-mp_3)^2}{2mp_3(1-p_3)}\bigg)+O(\frac{1}{\sqrt m})
\end{align*}
which implies the following
\begin{align*}
    \bfa P(\bfa X>\bfa Y,\bfa X>\bfa Z)&=\int_{-\infty}^\infty \bfa P(\bfa X=x)\bfa P(\bfa Y<x)\bfa P(\bfa Z<x)dx\\
    &=\sum_{i=1}^m\bigg[\bigg(\sum_{j=1}^{i-1}\binom{m}{j}p_2^j(1-p_2)^{m-j}\bigg)\bigg(\sum_{k=1}^{i-1}\binom{m}{j}p_3^k(1-p_3)^{m-k}\bigg)\bigg]\binom{m}{i}p_1^i(1-p_1)^{m-i}\\
    &\leq\sum_{i=1}^{m\lfloor\min(p_2,p_3)\rfloor}\binom{m}{i}p_1^i(1-p_1)^{m-i}\exp\bigg(-\frac{(i-mp_2)^2}{2mp_2(1-p_2)}-\frac{(i-mp_3)^2}{2mp_3(1-p_3)}\bigg)\\
    &+\sum_{i=\lceil m\min(p_3,p_2)\rceil}^{m\lfloor m\max(p_2,p_3)\rfloor}\binom{m}{i}p_1^i(1-p_1)^{m-i}\exp\bigg(-\frac{(i-m\max\{ p_2,p_3\})^2}{2m\max\{p_2,p_3\}(1-\max\{p_2,p_3\})}\bigg)\\
    &+\sum_{i=\lfloor m\max\{p_2,p_3\}\rfloor}^m\binom{m}{i}p_1^i(1-p_1)^{m-i}\\
    &\leq\sum_{i=1}^{m\lfloor\min(p_2,p_3)\rfloor}\binom{m}{i}p_1^i(1-p_1)^{m-i}\exp\bigg(-\frac{(i-mp_2)^2}{2mp_2(1-p_2)}-\frac{(i-mp_3)^2}{2mp_3(1-p_3)}\bigg)\\
    &+\sum_{i=\lfloor m\min(p_3,p_2)\rfloor}^m\binom{m}{i}p_1^i(1-p_1)^{m-i}
    \end{align*}
    where the last inequality comes from the fact that when $i\in\{\lfloor\min\{(p_2,p_3)\}\rfloor+1,\ldots,\lfloor\max\{(p_2,p_3)\}\rfloor\}$
    \begin{align*}
        \exp\bigg(-\frac{(y-m\max(p_2,p_3))^2}{2m\max\{p_2,p_3\}(1-\max\{p_2,p_3\})}\bigg)\leq 1
    \end{align*}
    We upperbound the $2$ terms seperately. Since we have $\min(p_2,p_3)>p_1$ the upperbound to the second term can be directly obtained by the Hoeffding's inequality, given by:
    \begin{align*}
        \sum_{i=\lfloor m\min(p_3,p_2)\rfloor}^m\binom{m}{i}p_1^i(1-p_1)^{m-i}&=\bfa P(\bfa X>\lfloor m\min(p_3,p_2)\rfloor)\\
        &\leq\exp(-\frac{(mp_1-m\lfloor\min(p_3,p_2)\rfloor)^2}{2mp_1(1-p_1)})+O(\frac{1}{\sqrt m})
    \end{align*}
    To upperbound the first term, we have
    \begin{align*}
    &\sum_{i=1}^{m\lfloor\min(p_2,p_3)\rfloor}\binom{m}{i}p_1^i(1-p_1)^{m-i}\exp\bigg(-\frac{(i-mp_2)^2}{2mp_2(1-p_2)}-\frac{(i-mp_3)^2}{2mp_3(1-p_3)}\bigg)\\
    % &\leq\sum_{i=1}^{m\lfloor\min(p_2,p_3)\rfloor}\frac{m^i\log^i(1-p_1)}{i!}\exp\bigg(-m\bigg(\log(1-p_1)+2\big((p_3-\frac{i}{m})^2+(p_2-\frac{i}{m})^2\big)\bigg)\bigg)\\
    % &\leq \int_{0}^{m\lfloor\min(p_2,p_3)\rfloor}\frac{1}{\sqrt{2\pi mp_1(1-p_1)}}\exp\bigg(-\frac{(x-mp_1)^2}{2mp_1(1-p_1)}-2m\big((p_3-\frac{x}{m})^2+(p_2-\frac{x}{m})^2\big)\bigg)dx+O(\frac{\exp(-Cm^2)}{\sqrt{m}})\\
    &\leq \int_{0}^{m\lfloor\min(p_2,p_3)\rfloor}\frac{1}{\sqrt{2\pi mp_1(1-p_1)}}\exp\bigg(-\frac{(x-mp_1)^2}{2mp_1}-\frac{(x-mp_2)^2}{2mp_2(1-p_2)}-\frac{(x-mp_3)^2}{2mp_3(1-p_3)}\bigg)dx\\
    &+O(\frac{\exp(-Cm^2)}{\sqrt{m}})\\
    &=\int_{0}^{m\lfloor\min(p_2,p_3)\rfloor}(2\pi mp_1(1-p_1))^\frac{-1}{2}\exp-\bigg(\frac{1+8p_1(1-p_1)}{2mp_1(1-p_1)}x^2+(-1-2p_3-2p_2)x+m(\frac{1}{2}p_1^2+2p_2^2+2p_3^2)\bigg)dx\\
    &+O(\frac{\exp(-Cm^2)}{\sqrt{m}})\\
    &=( mp_1(1-p_1))^{-\frac{1}{2}}\exp-\bigg(m(\frac{1}{2}p_1^2+2p_2^2+2p_3^2)-\frac{(-1-2p_3-2p_2)^2}{4\frac{1+8p_1(1-p_1)}{2mp_1(1-p_1)}}\bigg)+O(\frac{\exp(-Cm^2)}{\sqrt{m}})\\
    &\int_{0}^{m\lfloor\min(p_2,p_3)\rfloor}\frac{1}{\sqrt{2\pi}}\exp-\frac{1+8p_1(1-p_1)}{2mp_1(1-p_1)}\bigg(x+\frac{-1-2p_3-2p_2}{2\frac{1+8p_1(1-p_1)}{2mp_1(1-p_1)}}\bigg)^2dx+O(\frac{\exp(-Cm^2)}{\sqrt{m}})\\
    &= (1+8p_1(1-p_1))^{-\frac{1}{2}}\exp-\bigg(m(\frac{1}{2}p_1^2+2p_2^2+2p_3^2)-\frac{(-1-2p_3-2p_2)^2}{4\frac{1+8p_1(1-p_1)}{2mp_1(1-p_1)}}\bigg)\\
    &(\Phi(A(m))-\Phi(B(m)))+O(\frac{\exp(-Cm^2)}{\sqrt{m}})\\
    &\leq(1+8p_1(1-p_1))^{-\frac{1}{2}}\exp-\bigg(m(\frac{1}{2}p_1^2+2p_2^2+2p_3^2)-\frac{(-1-2p_3-2p_2)^2}{4\frac{1+8p_1(1-p_1)}{2mp_1(1-p_1)}}\bigg)+O(\frac{\exp(-Cm^2)}{\sqrt{m}})
    \end{align*}
    where $\Phi(x)=\bfa P(X\leq x)$ where $X\sim N(0,1)$ and we immediately have
    \begin{align*}
        \Phi(x_1)-\Phi(x_2)\leq 1
    \end{align*}
    which completes the estimate.
%     &\leq \int_{0}^m(2\pi mp_1)^{-\frac{1}{2}}\bigg(\frac{(x-mp_1)^2}{2mp_1}+2m\big((p_3-\frac{x}{m})^2+(p_2-\frac{x}{m})^2\big)\bigg)^{-1}dx\\
%     &=\int_{0}^m(2\pi mp_1)^{-\frac{1}{2}}\bigg(\frac{1+8p_1(1-p_1)}{2mp_1(1-p_1)}x^2+(-1-2p_3-2p_2)x+m(\frac{1}{2}p_1^2+2p_2^2+2p_3^2)\bigg)
% \end{align*}
% We know that when $ax^2+bx+c>0$ for all $x$ $(4ac-b^2>0)$, the integral yield the following:
% \begin{equation*}
%     \int \frac{1}{ax^2+bx+c}dx=\frac{1}{\sqrt{b^2-4ac}}\ln\bigg|\frac{2ax+b-\sqrt{b^2-4ac}}{2ax+b+\sqrt{b^2+4ac}}\bigg|+k
% \end{equation*}
\end{proof}
\begin{lemma}\label{lm11}
Let $\bfa X\sim Binom(m,p_1),\bfa Y\sim Binom(m,p_2),\bfa Z\sim Binom(m,p_3)$. Assuming $p_1\leq\min(1-p_2,p_3)$ then  \begin{align*}
    \bfa P(\bfa Y>\bfa X>\bfa Z)&\leq(1+8p_1(1-p_1))^{-\frac{1}{2}}\exp\bigg(-m(\frac{1}{2}p_1^2+2(1-p_2)^2+2p_3^2)\\
    &+\frac{(-1-2p_3-2(1-p_2))^2}{4\frac{1+8p_1(1-p_1)}{2mp_1(1-p_1)}}\bigg)
\end{align*}when $m$ is large but not necessarily going to infinity.
\end{lemma}
\begin{proof}
Similar to the proof of lemma \ref{lm10}, we start by writing it as an integral. In particular, we observed that by replacing $p_2$ in Lemma \ref{lm10} by $1-p_2$, we will obtain the proof. The details is stated by
\begin{align*}
\bfa P(\bfa Y>\bfa X>\bfa Z)&=\int_{-\infty}^\infty\bfa P(\bfa Y >x)\bfa P(\bfa X=x)\bfa P(
\bfa Z<x)dx\\
&=\sum_{i=1}^m\bigg[\bigg(\sum_{j=i}^m\binom{m}{j}p_2^j(1-p_2)^{m-j}\bigg)\bigg(\sum_{k=1}^{i-1}\binom{m}{j}p_3^k(1-p_3)^{m-k}\bigg)\bigg]\binom{m}{i}p_1^i(1-p_1)^{m-i}
% &\leq\sum_{i=1}^m\binom{m}{i}p_1^i(1-p_1)^{m-i}\exp\bigg(-2m\big ((p_2-\frac{m-i}{m})^2+(p_2-\frac{i}{m})^2\big )\bigg)\\
% &\leq\int_{0}^m\frac{1}{\sqrt{2\pi mp_1}}\exp\bigg(-\frac{(x-mp_1)^2}{2mp_1}-2m\big ((p_2-\frac{m-i}{m})^2+(p_2-\frac{i}{m})^2\big )\bigg)dx\\
% &=(2\pi m p_1)^{-\frac{1}{2}}\int_{0}^m\exp\bigg(-\frac{(x-mp_1)^2}{2mp_1}-2m\big((p_2-\frac{m-i}{m})^2+(p_2-\frac{i}{m})^2\big)\bigg)dx\\
% &\leq(4p_1+1)^{-\frac{1}{2}}\exp-\bigg(m(\frac{1}{2}p_1^2+2(1-p_2)^2+2p_3^2)-\frac{-1-2p_3-2(1-p_2))^2}{2\frac{4p_1+1}{mp_1}}\bigg)
\end{align*}
where the argument follows exactly from the previous lemma.
\end{proof}
% For the joint event over $4$ indices, the following should hold:
% \begin{lemma}
% Let $\bfa X\sim Binom(m,p_1)$, $\bfa Y\sim Binom(m,p_2)$, $\bfa Z\sim Binom(m,p_3)$ and $\bfa W\sim Binom(m,p_4)$ and independent. Assume that $p_1<\min(p_2,p_3)<\max(p_2,p_3)<p_4$ and $m$ is large, then $\bfa P(\bfa X>\min(\bfa Y,\bfa Z)\geq\max(\bfa Y,\bfa Z)>\bfa W)$ 
% \end{lemma}
% \begin{proof}
% We adopt similar method as proving the previous two lemmas. We cannot directly use tailbound but use the fact that $Binom(m,p)$ is dominated by $\ca N(mp,mp)$ when $m$ is very large.
% \begin{align*}
%     &\bfa P(\bfa X>\max(\bfa Y,\bfa Z)\geq\min(\bfa Y,\bfa Z)>\bfa W)\\
%     &=\sum_{i=2}^{m}\binom{m}{i}p_1^i(1-p_1)^{m-i}\sum_{l=i-2}^{m-2}\binom{m}{l}p_4^i(1-p_4)^{m-i}\bigg(\sum_{j=i+1}^{l-1}\binom{m}{j}p_2^l(1-p_2)^{m-l}\bigg)\\
%     &\bigg(\sum_{k=i+1}^{l-1}\binom{m}{k}p_3^k(1-p_3)^{m-k}\bigg)\\
%     &\int_{}
% \end{align*}
% \end{proof}
Then the following theorem gives the impossibility condition according to lemma \ref{lm1}.
\begin{theorem}
Let $\Delta=\sum_{k\in[n]\setminus\{a,b\}}| M_{a,k}-M_{b,k}|$. Assuming that $m$ is sufficiently large. Then the following implies impossibility.
\begin{align*}
    \Delta\leq\sqrt{\frac{\log n}{mn}+\frac{\log(8\gamma_{\min}(1-\gamma_{\min})+1)}{m}+\frac{2K}{n}}
\end{align*}
with 
\begin{align*}
    K&=\inf_{i,j,k}\sum_{o\in[n]\setminus\{i,j,k\}}\bigg(\frac{1}{2}M_{k,o}^2+2M_{j,o}^2+2M_{i,o}^2-\frac{M_{k,o}}{2(8M_{k,o}(1-M_{k,o})+1)}\big(1+2M_{k,o}+2M_{o,i}\big)^2\bigg)\\
    \gamma_{\min}&=\inf_{i,j}M_{i,j}
\end{align*}
\end{theorem}
\begin{proof}
Let $(a,b)=\argmin_{(i,j)}\bfa P_{i,j}$. We then use the independence condition, lemma \ref{lm:88}, note that $\bfa X_{a,k}\sim Binom(m, M_{a,k})$ and $\bfa X_{b,k}\sim Binom(m,M_{b,k})$, by Hoeffding's inequality, we have
\begin{align*}
\bfa P(F_{a,b})&=\prod_{k\in[n]\setminus\{a,b\}}\bfa P(\bfa X_{a,k}>\bfa X_{b,k})\\
&=\prod_{k\in[n]\setminus\{a,b\}}\bfa P\bigg(\bfa X_{b,k}-\bfa X_{a,k}-\bb E[\bfa X_{b,k}-\bfa X_{a,k}]<-\bb E[\bfa X_{b,k}-\bfa X_{a.k}]\bigg)\\
&\geq\prod_{k\in[n]\setminus\{a,b\}}\exp\bigg(-\frac{m(M_{a,k}-M_{b,k})^2}{2}\bigg)\\
&=\exp\bigg(\sum_{k\in[n]\setminus\{a,b\}}-\frac{m(M_{a,k}-M_{b,k})^2}{2}\bigg)
% \leq \prod_{k\in[n]\setminus\{a,b\}}\exp\bigg(-2\bigg(\frac{M_{b,k}(1-M_{a,k})}{M_{a,k}(1-M_{b,k})+M_{b,k}(1-M_{a,k})} - \frac 12\bigg)^2\\& \big(M_{a,k}(1-M_{b,k}) + M_{b,k}(1-M_{a,k})\big) m\bigg)\\
% &\leq\exp\bigg(\frac{\sum_{k=1}^n m(M_{a,k}-M_{b,k})^2}{2}\bigg)
\end{align*}
And we let $x_{i,j,o}=\sqrt{\frac{m(M_{j,o}-M_{i,o})^2}{M_{j,o}(1-M_{j,o})+M_{i,o}(1-M_{i,o})}}$ and have
\begin{align*}
    \mu_n^2&:=\bigg(\sum_{i<j}\bfa P(F_{i,j})\bigg)^2\geq\bigg ( \sum_{i<j}\prod_{o\in[n]\setminus\{i,j\}}\bigg (\frac{1}{x_{i,j,o}}-\frac{1}{x_{i,j,o}^3}\bigg )\exp\bigg (-\frac{x_{i,j,o}^2}{2}\bigg )\bigg )^2
\end{align*}
Then we see the following joint events $F_{i,j}\cap F_{j,k}$ between on $i,j,k$ with $i<j<k$
\begin{equation*}
    \left\{\begin{matrix}
F_{i,j}\cap F_{j,k}: &\bfa X_{i,k}>\bfa X_{j,k} \text{ and }\bfa X_{j,i}>\bfa X_{k,i} \text{ and }\bfa X_{i,o}>\bfa X_{j,o}>\bfa X_{k,o} \text{ for all }o\in[n]\setminus\{i,j,k\}\\
F_{i,k}\cap F_{j,k}: & \bfa X_{i,j}>\bfa X_{k,j}\text{ and } \bfa X_{j,i}>\bfa X_{k,i}\text{ and }\bfa X_{i,o}>\bfa X_{k,o},\bfa X_{j,o}>\bfa X_{k,o} \text{ for all }o\in[n]\setminus\{i,j,k\} \\
\end{matrix}\right.
\end{equation*}
By lemma \ref{lm11}, we get that
\begin{align*}
    &\bfa P\bigg(F_{i,j}\cap F_{j,k}\bigg)=\bfa P\bigg( \bfa X_{i,j}>\bfa X_{i,k}>\bfa X_{j,k}\bigg)\cdot\prod_{o\in [n]\setminus\{i,j,k\}}\bfa P\bigg (\bfa X_{i,o}>\bfa X_{j,o}>\bfa X_{k,o}\bigg )\\
    &\leq (1+8M_{i,k}(1-M_{i,k}))^{-\frac{1}{2}}\exp\bigg(-m(\frac{1}{2}M_{i,k}^2+2(1-M_{i,j})^2+2M_{j,k}^2)+\frac{(-1-2M_{j,k}-2(1-M_{i,j}))^2}{4\frac{1+8M_{i,k}(1-M_{i,k})}{2mM_{i,k}}}\bigg)\\
    &\cdot\prod_{o\in[n]\setminus\{i,j,k\}} (1+8M_{j,o}(1-M_{j,o}))^{-\frac{1}{2}}\exp\bigg(-m(\frac{1}{2}M_{j,o}^2+2(1-M_{i,o})^2+2M_{k,o}^2)\\&
    +\frac{(-1-2M_{k,o}-2(1-M_{i,o}))^2}{4\frac{8M_{j,o}(1-M_{j,o})+1}{2mM_{j,o}}}\bigg)\\
    &\leq\bigg(\prod_{o\in[n]\setminus\{i,j,k\}}(1+8M_{j,o}(1-M_{j,o}))\bigg)^{-\frac{1}{2}}\exp\bigg(-m\sum_{o\in[n]\setminus\{i,j,k\}}\bigg(\frac{1}{2}M_{j,o}^2+2M_{o,i}^2+2M_{k,o}^2\\
    &-\frac{M_{j,o}}{2(8M_{k,o}(1-M_{k,o})+1)}\big(1+2M_{k,o}+2M_{o,i}\big)^2\bigg)\bigg)
\end{align*}
For the second regime, we can upperbound the probability of joint event with lemma \ref{lm10}. 
\begin{align*}
    &\bfa P(F_{i,k}\cap F_{j,k})=\bfa P(\bfa X_{i,j}>\bfa X_{k,j}\text{ and } \bfa X_{i,j}>\bfa X_{i,k})\cdot\prod_{o\in[n]\setminus\{i,j,k\}}\bfa P(\bfa X_{o,k}>\max(\bfa X_{o,i},\bfa X_{o,j}))\\
     &\leq (1+8M_{i,j}(1-M_{i,j}))^{-\frac{1}{2}}\exp\bigg(-m(\frac{1}{2}M_{i,j}^2+2M_{k,j}^2+2M_{i,k}^2)+\frac{(-1-2M_{k,j}-2M_{i,k})^2}{4\frac{1+8M_{i,j}(1-M_{i,j})}{2mM_{i,j}}}\bigg)\\
    &\cdot\prod_{o\in[n]\setminus\{i,j,k\}} (8M_{k,o}(1-M_{k,o})+1))^{-\frac{1}{2}}\exp\bigg(\bigg(-m(\frac{1}{2}M_{o,k}^2+2M_{o,i}^2+2M_{o,j}^2)\\&
    +\frac{(-1-2M_{k,o}-2(1-M_{i,o}))^2}{4\frac{(8M_{k,o}(1-M_{k,o})+1))}{2mM_{k,o}}}\bigg)+\exp(-2m(M_{o,k}-\lfloor\min(M_{o,j},M_{o,i})\rfloor)^2)\bigg)\\
    &\leq\bigg(\prod_{o\in[n]\setminus\{i,j,k\}}(8M_{k,o}(1-M_{k,o})+1)\bigg)^{-\frac{1}{2}}\exp\bigg(-m\sum_{o\in[n]\setminus\{i,j,k\}}\bigg(\frac{1}{2}M_{k,o}^2+2M_{j,o}^2+2M_{i,o}^2\\
    &-\frac{M_{k,o}}{2(8M_{k,o}(1-M_{k,o})+1)}\big(1+2M_{k,o}+2M_{o,i}\big)^2\bigg)\bigg)
\end{align*}
Where in the last inequality we used the fact that $\exp(-mC)\rightarrow 0$ as $m\rightarrow\infty$ for positive $C$.
Then we also give the joint events induced by $4$ complete discrete indices $i,j,k,l$ with $i<j<k<l$. For simplicity, we omit the duplicate term in $[n]\setminus\{i,j,k,l\}$ and only give the possible relationship between those $4$ indices here.
\begin{equation*}
    \left\{\begin{matrix}
F_{i,j}\cap F_{k,l}: &\bfa X_{i,l}>\bfa X_{j,l}>\bfa X_{j,k}\text{ and }\bfa X_{i,l}>\bfa X_{i,k}>\bfa X_{j,k}\\
F_{i,l}\cap F_{j,k}: & \bfa X_{i,k}>\bfa X_{i,j}>\bfa X_{l,j}\text{ and }\bfa X_{i,k}>\bfa X_{l,k}>\bfa X_{l,j}\\
F_{i,k}\cap F_{j,l}:&\bfa X_{i,l}>\bfa X_{i,j}>\bfa X_{k,j}\text{ and }\bfa X_{i,l}>\bfa X_{k,l}>\bfa X_{k,j}
\end{matrix}\right.
\end{equation*}
Although these events is connecting $4$ indices in the graph, the multiplicity is always $1$ , which implies that they can be ignored. Henceforth, the only term we need to consider is in the following form, where we take the first case as an example
\begin{align*}
    \bfa P(F_{i,j}\cap F_{k,l})&=\bfa P(\bfa X_{i,l}>\max(\bfa X_{j,l},\bfa X_{i,k})>\bfa X_{j,k})\cdot\prod_{o\in[n]\setminus\{i,j,k,l\}}\bfa P(\bfa X_{i,o}<\bfa X_{j,o},\bfa X_{k,o}<\bfa X_{l,o})\\
    &\leq\prod_{o\in[n]\setminus\{i,j,k,l\}}\bfa P(\bfa X_{i,o}<\bfa X_{j,o})\cdot\bfa P(\bfa X_{k,o}<\bfa X_{l,o})=\bfa P(F_{i,j})\cdot\bfa P(F_{k,l})
    \end{align*}
Collecting pieces, we get
\begin{align*}
    \gamma_n&\leq\sum_{i,j,k,l\in[n]}\bfa P(F_{i,j})\cdot\bfa P(F_{k,l})+\sum_{i,j,k\in[n]}\bigg(\prod_{o\in[n]\setminus\{i,j,k\}}(8M_{k,o}(1-M_{k,o})+1)\bigg)^{-\frac{1}{2}}\\
    &\exp\bigg(-m\sum_{o\in[n]\setminus\{i,j,k\}}\bigg(\frac{1}{2}M_{k,o}^2+2M_{j,o}^2+2M_{i,o}^2-\frac{M_{k,o}}{2(8M_{k,o}(1-M_{k,o})+1)}\big(1+2M_{k,o}+2M_{o,i}\big)^2\bigg)\bigg)
    % \\
    % &\leq\sum_{i,j,k,l\in[n]}\bfa P(F_{i,j})\cdot\bfa P(F_{k,l})+\sum_{i,j,k\in[n]}\bigg(\prod_{o\in[n]\setminus\{i,j,k\}}(8M_{k,o}(1-M_{k,o})+1)\bigg)^{-\frac{1}{2}}\\
    % &\exp\bigg(-m\sum_{o\in[n]\setminus\{i,j,k\}}\bigg)
\end{align*}
Note that by corollary~\ref{cor1.2}, we have
\begin{align*}
    \bfa P\bigg (\bigcup_{i<j}F_{i,j}\bigg )\geq\frac{1}{1+\frac{1}{\mu_n}+\frac{\gamma_n}{\mu_n^2}}
\end{align*}$\sum_{i,j,k,l\in[n]}\bfa P(F_{i,j})\cdot\bfa P(F_{k,l})=O(\mu_n^2)$. Let $\gamma_n=O(\mu_n^2)$ and obtain the final result.
\end{proof}


==> sections/minimax.tex <==
Here we discuss the Minimax rate of this problem. Instead of using $0/1$ loss as in the requirement of exact recovery, we use KL loss, which is stated as
\begin{align*}
    \bb E_{M,\Pi}D_\text{KL}(\pi\Vert\wh\pi)=\int D_\text{KL}(\bfa P(\cdot|\Pi=\pi)\Vert \bfa P(\cdot|\Pi=\wh\pi(\bfa A_1^m))\bfa P(d\bfa A_1^m)
\end{align*}
And the minimax risk with regard to some matrix $M$ is
\begin{align*}
    \inf_{\wh\Pi}\sup_{\Pi\in\ca P}\bb E_{M,\Pi}D_\text{KL}(\pi\Vert\wh\pi)
\end{align*}
In the previous work ~\citep{shah2017simple}, a result for Minimax lower bound is obtained, which is stated as:
\begin{theorem}{~\citep{shah2017simple}}
If $M$ satisfy the following condition, then there exists at least a single $M$ that cannot be exactly ranked:
\begin{align*}
    \bar\Delta\leq\frac{1}{70}\sqrt{\frac{\log n}{mnp}}
\end{align*}
\end{theorem}
Before we state the main result, we will need the following technical lemma regarding the metric entropy with KL distance
\begin{definition}[Metric Entropies of KL Divergence]
Let $\ca N(\ca P, d_\text{KL},\epsilon)$ be the $\epsilon$-covering of bijection family $\ca P$. Then for all $\pi\in\ca P$, there exists $\pi_i\in\ca N(\ca P,d_\text{KL},\epsilon)$ such that
\begin{align*}
    D_\text{KL}( \pi\Vert \pi_i)\leq \epsilon
\end{align*}
Similarly, let $\ca M(\ca P,d_\text{KL})$ be the $\epsilon$-packing of bijection family $\ca P$. Then for any , there exists $\pi_i\in\ca M(\ca P,d_\text{KL},\epsilon)$ such that

\begin{align*}
    N(\ca P,\epsilon)=|\ca N(\ca P,d_\text{KL},\epsilon)|\leq 
\end{align*}
\end{definition}
% \begin{proof}
% Let $\ca M(\ca P,d_\text{KL},\epsilon)$ be the $\epsilon$-packing of a bijection family $\ca P$. Let $M(\ca P, d_\text{KL},\epsilon)=|\ca M(\ca P, d_\text{KL},\epsilon)|$ be the $\epsilon$-packing number. Moreover, we note that the set $|\ca P|=n!$, 
% \end{proof}
And we have the following result regarding the Minimax upper bound
\begin{theorem}
If $M$ satisfies the following condition, then there exists at least a single $M$ that can be exactly ranked:
\end{theorem}
\begin{proof}
The minimax upperbound relies on the technique introduced in~\citet{yang1999information}. We consider the following estimate:
\begin{align*}
    \bfa P(\bfa A_{m+1}=A|\wh\pi(\bfa A_1^m))=\frac{1}{m}\sum_{i=0}^{m-1}\bfa P(\bfa A_{i+1}=A|\bfa A_1^i)
\end{align*}
with
\begin{align*}
    \bfa P(\bfa A_i|\bfa A_1^i)=\frac{\int \fk P(d\pi)\prod_{j=1}^i\bfa P(\bfa A_j|\pi)}{\int\fk P(d\pi)\prod_{j=1}^{i-1}\bfa P(\bfa A_j|\pi)}
\end{align*}
With an appropriate prior $\fk P$, we see that
\begin{align*}
     D_\text{KL}(\pi\Vert\wh\pi)&=D_\text{KL}\bigg (\bfa P(\bfa A|\pi)\Big\Vert\frac{1}{m}\sum_{i=0}^{m-1}\bfa P(\bfa A_{i+1}|\bfa A_1^i)\bigg)\\
    &\leq\frac{1}{m}\sum_{i=0}^{m-1}\dkl\bigg(\bfa P(\bfa A|\pi)\Big\Vert\frac{1}{m}\sum_{i=0}^{m-1}\bfa P(\bfa A_{i+1}|\bfa A_1^i)\bigg)\\
    &=\frac{1}{m}D_\text{KL}\bigg(\bfa P(\bfa A_1^m|\pi)\Big\Vert\bfa P(\bfa A_1^m)\bigg)
    % &=\frac{1}{m}\sum_{i,j\in[n]:i<j}\dkl\bigg(\bfa P(\bfa A_{1,i,j}^m|\pi)\Big\Vert\frac{1}{}\bfa P()\bigg)
\end{align*}
where the inequality comes from the convexity of KL divergence and the equality comes from the the tensorization of KL divergence.

Consider a cover $\ca N(\ca P,d_\text{KL},\epsilon)$ with $N=|\ca N(\ca P,d_\text{KL},\epsilon)|$, choose $\fk P(\Pi)\sim\text{ Uniform }(\ca N)$.
Without loss of generality, we denote the cover by $\ca N$ in the sequel. We also define the following statement :
\begin{align*}
    \pi_i(\pi)=\argmin_{\pi^\prime\in\ca N}\dkl(\pi\Vert\pi^\prime)\leq\epsilon
\end{align*}
then the following holds:
\begin{align*}
    \dkl\bigg(\bfa P(\bfa A_1^m|\pi)\Big\Vert \bfa P(\bfa A_1^m)\bigg)&=\dkl\bigg(\bfa P(\bfa A_1^m|\pi)\Big\Vert\bfa P(\bfa A_1^m)\bigg)\\
    % &=\sum_{i<j:i,j\in[n]}\dkl\bigg(\bfa P(\bfa A_{1,i,j}^m|\pi)\Big\Vert\bfa P(\bfa A_{1,i,j}^m)\bigg)\\
    % &=\sum_{i<j:i,j\in[n]}\dkl\bigg(\bfa P(\bfa A_{1,i,j}^m|\pi)\Big\Vert\frac{1}{n!}\sum_{\pi\in\ca P}\bfa P(\bfa A_{1,i,j}^m|\pi)\bigg)\\
    % &=
    &=\bb E\log\bigg[\frac{\bfa P(\bfa A_1^m|\pi)}{\frac{1}{N}\sum_{\pi_i\in\ca N}\bfa P(\bfa A_1^m|\pi_i)}\bigg]\\
    &\leq \bb E\log\bigg[\frac{\bfa P(\bfa A_1^m|\pi)}{\frac{1}{N}\bfa P(\bfa A_1^m|\pi_i(\pi))}\bigg]\\
    &\leq\log N+ m\epsilon
\end{align*}
This gives us the upper bound on the Minimax risk
\begin{align*}
    \inf_{\wh\pi}\sup_{\pi\in\ca P}\bb E_{M,\pi}\dkl(\pi\Vert\wh\pi)\leq\sup_{\pi\in\ca P}\bb E_{M,\pi} \dkl(\pi\Vert\wh\pi)\leq \frac{1}{m}\log N+\epsilon
\end{align*}
The next step is to upperbound the covering number of $\ca P$ with the metric defined by KL loss. By Stirling's approximation, we see that
\begin{align*}
    \log|\ca P|=n\log n +o(n\log n)
\end{align*}
Take $\epsilon=\inf_{\pi,\pi^\prime} D_\text{KL}(\pi\Vert\pi^\prime)$, and use the duality between packing and covering number, we see that
\begin{align*}
    
\end{align*}
\end{proof}

